Approaching Human-Level Forecasting with Language Models

Forecasting future events is important for policy and decision making. In this work, we study whether language models (LMs) can forecast at the level of competitive human forecasters. Towards this goal, we develop a retrieval-augmented LM system designed to automatically search for relevant information, generate forecasts, and aggregate predictions. To facilitate our study, we collect a large dataset of questions from competitive forecasting platforms. Under a test set published after the knowledge cut-offs of our LMs, we evaluate the end-to-end performance of our system against the aggregates of human forecasts. On average, the system nears the crowd aggregate of competitive forecasters, and in some settings surpasses it. Our work suggests that using LMs to forecast the future could provide accurate predictions at scale and help to inform institutional decision making.

==> figures/3_plots.tex <==
\begin{figure}[!t]
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{plots/calibration_plot.pdf}
        \caption{Calibration of our system vs crowd.}
        \label{fig:calibration}
    \end{subfigure}
    \hfill % This command adds space between the subfigures if needed
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{plots/distribution_of_predictions.pdf}
        \caption{Distribution of predictions.}
        \label{fig:prediction_distributions}
    \end{subfigure}
    \hfill % This command adds space between the subfigures if needed
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth]{plots/brier_scores_over_retrieval_dates.pdf}
        \caption{Brier score over retrieval indices.}
        \label{fig:brier_score_over_dates}
    \end{subfigure}
    \caption{\textbf{(a)} Our system is well calibrated on the test set. \textbf{(b)} The crowd outperforms us on questions where they confidently predict ``No''. \textbf{(c)} Our system's Brier score does not decline at the same rate as the crowd's as the question comes close to resolution, suggesting opportunities to improve our retrieval system.}
    \label{fig:3_plots}
\end{figure}

==> figures/calibration_plot_test_wrap.tex <==
\begin{wrapfigure}{r}{0.4\textwidth}
\vspace{-1em}
  \centering
    \includegraphics[width=0.4\textwidth]{plots/calibration_plot.pdf}
    \caption{\textbf{Our system is well calibrated at test time.} The crowd is also well calibrated, as it was before on earlier questions (c.f. \autoref{fig:calibration_validation}).}
    \label{fig:calibration_test}
    \vspace{-4.0em}
\end{wrapfigure}
% --

==> figures/calibration_plot_validation_wrap.tex <==
\begin{wrapfigure}{r}{0.4\textwidth}
\vspace{-2.4em}
  \centering
    \includegraphics[width=0.4\textwidth]{plots/calibration_plot_validation.pdf}
    \caption{\textbf{Our system is well calibrated.} The crowd is also well calibrated, consistent with \citet{zou2022forecasting}'s findings.}
    \label{fig:calibration_validation}
    \vspace{-4.0em}
\end{wrapfigure}
% --

==> figures/news_apis_relevancy.tex <==
\begin{figure}[ht]
  \centering
  \includegraphics[width=0.6\linewidth]{plots/relevancy_scores_by_news_api.pdf}
  \caption{
    \textbf{Relevance scores of articles retrieved via news APIs.} 
  }
  \label{fig:news-api-relevance}
\end{figure}


==> tables/base_eval_knowledge_by_set.tex <==
\begin{table}[h!]
  \centering
  \small
  \begin{tabular}{@{}l r r r r r r@{}}
    \toprule
    & \multicolumn{3}{c}{\textbf{Train (Before Cut-off)}} & \multicolumn{3}{c}{\textbf{Test (After Cut-off)}} \\
    \cmidrule(lr){2-4} \cmidrule(lr){5-7}
    \textbf{Model} & \textbf{Percent Correct} & \textbf{Percent Incorrect} & \textbf{Percent IDK/Other} & \textbf{Percent Correct} & \textbf{Percent Incorrect} & \textbf{Percent IDK/Other} \\
    \midrule
    GPT-3.5-Turbo & 0.343 & 0.314 & 0.342 & 0.272 & 0.239 & 0.489 \\
    GPT-3.5-Turbo-1106 & 0.238 & 0.219 & 0.543 & 0.144 & 0.146 & 0.709 \\
    GPT-4 & 0.203 & 0.023 & 0.774 & 0.001 & 0.0 & 0.999 \\
    GPT-4-1106-Preview & 0.24 & 0.02 & 0.741 & 0.001 & 0.0 & 0.999 \\
    LLama-2-7B & 0.067 & 0.102 & 0.831 & 0.022 & 0.028 & 0.95 \\
    LLama-2-13B & 0.196 & 0.102 & 0.703 & 0.068 & 0.043 & 0.89 \\
    LLama-2-70B & 0.193 & 0.129 & 0.678 & 0.043 & 0.032 & 0.926 \\
    Mistral-7B-Instruct & 0.029 & 0.045 & 0.926 & 0.024 & 0.02 & 0.956 \\
    Mistral-8x7B-Instruct & 0.048 & 0.047 & 0.904 & 0.011 & 0.01 & 0.979 \\
   Mixtral-8x7B-DPO & 0.04 & 0.016 & 0.943 & 0.002 & 0.001 & 0.997 \\
    Yi-34B-Chat & 0.611 & 0.272 & 0.117 & 0.428 & 0.224 & 0.348 \\
    Claude-2 & 0.298 & 0.118 & 0.585 & 0.044 & 0.024 & 0.932 \\
    Claude-2.1 & 0.298 & 0.117 & 0.585 & 0.042 & 0.024 & 0.934 \\
    Gemini-Pro & 0.4 & 0.112 & 0.487 & 0.311 & 0.121 & 0.567 \\
    \bottomrule
  \end{tabular}
  \caption{\textbf{Model Knowledge Evaluation}: Comparative knowledge evaluation of various models in terms of correct, incorrect, and IDK/other responses across training \& validation, and test datasets.}
  \label{tab:model_performance}
\end{table}


==> tables/base_eval_knowledge_by_year.tex <==
\begin{table}[h!]
  \centering
  \small
  \begin{tabular}{@{}l r r r r r@{}}
    \toprule
    \textbf{Model} & \textbf{2015--2020} & \textbf{2021} & \textbf{2022} & \textbf{2023 (before Apr 1)} & \textbf{2023 (after Apr 1)} \\
    \midrule
    GPT-3.5-Turbo & 0.468 (0.016) & 0.534 (0.003) & 0.26 (0.001) & 0.251 (0.001) & 0.163 (0.001) \\
    GPT-3.5-Turbo-1106 & 0.479 (0.014) & 0.49 (0.003) & 0.456 (0.001) & 0.432 (0.001) & 0.483 (0.001) \\
    GPT-4$^\dagger$ & 0.752 (0.010) & 0.725 (0.002) & 0.136 (0.001) & 0.01 (0.0) & 0.0 (0.0) \\
    GPT-4-1106-Preview & 0.789 (0.010) & 0.798 (0.002) & 0.708 (0.001) & 0.483 (0.001) & 0.301 (0.001) \\
    LLama-2-7B & 0.284 (0.017) & 0.277 (0.002) & 0.202 (0.001) & 0.217 (0.001) & 0.179 (0.001) \\
    LLama-2-13B & 0.455 (0.015) & 0.521 (0.003) & 0.598 (0.001) & 0.632 (0.001) & 0.586 (0.001) \\
    LLama-2-70B & 0.499 (0.014) & 0.503 (0.003) & 0.465 (0.001) & 0.455 (0.001) & 0.498 (0.001) \\
    Mistral-7B-Instruct & 0.251 (0.017) & 0.332 (0.002) & 0.163 (0.001) & 0.121 (0.001) & 0.073 (0.001) \\
    Mistral-8x7B-Instruct & 0.324 (0.015) & 0.393 (0.003) & 0.243 (0.001) & 0.155 (0.001) & 0.169 (0.001) \\
    Mixtral-8x7B-DPO & 0.403 (0.014) & 0.495 (0.003) & 0.494 (0.001) & 0.483 (0.001) & 0.481 (0.001) \\
    YI-34B-Chat & 0.374 (0.014) & 0.427 (0.003) & 0.392 (0.001) & 0.332 (0.001) & 0.381 (0.001) \\
    Claude-2 & 0.287 (0.017) & 0.359 (0.003) & 0.36 (0.001) & 0.137 (0.001) & 0.166 (0.001) \\
    Claude-2.1 & 0.286 (0.017) & 0.359 (0.003) & 0.361 (0.001) & 0.137 (0.001) & 0.169 (0.001) \\
    Gemini-Pro & 0.447 (0.015) & 0.597 (0.003) & 0.543 (0.001) & 0.517 (0.001) & 0.412 (0.001) \\
    \bottomrule
  \end{tabular}
  \caption{\textbf{Knowledge accuracy}: The knowledge accuracy of all $13$ language models from 2015 to 2023, including accuracy values and 2 standard errors (SE). $^\dagger$For almost all questions in  2023, GPT-4 correctly answers our knowledge  prompts by ``I don't know'', leading to (near) zero accuracy.}
  \label{tab:yearly_performance} 
\end{table}

==> tables/base_eval_short.tex <==
\begin{wraptable}{r}{0.5\textwidth} 
\vspace{-1.1em}
\begin{tabular}{@{}l r r@{}}
    \toprule
    \textbf{Model} & \textbf{Zero-shot} & \textbf{Scratchpad} \\
    \midrule
    GPT-4-1106-Preview & $\mathbf{0.208}$ $(0.006)$ & $\mathbf{0.209}$ $(0.006)$ \\
    Llama-2-13B & $0.226$ $(0.004)$ & $0.268$ $(0.004)$ \\
    Mistral-8x7B-Instruct & $0.238$ $(0.009)$ & $0.238$ $(0.005)$ \\
    Yi-34B-Chat & $0.238$ $(0.006)$ & $0.241$ $(0.004)$ \\
    Claude-2.1 & $0.220$ $(0.006)$ & ${0.215}$ $(0.007)$ \\
    Gemini-Pro & $0.243$ $(0.009)$ & ${0.230}$ $(0.003)$ \\
    \hline
    Trimmed Mean & $0.208$ $(0.006)$ & $0.224$ $(0.003)$ \\
    \bottomrule
  \end{tabular}
  \caption{\textbf{Zero-shot and scratchpad scores} of the best model in each series on the test set, with $1$ standard error (SE) (see full results in \autoref{tab:model_comparison}). Ensemble takes the trimmed mean using the best models from each series. Random baseline: 0.250; human crowd: 0.149 (averaged across all crowd predictions).}
  \label{tab:model_comparison_short} 
  \vspace{-0.5em}
\end{wraptable}


==> tables/train_test_distribution_wrap.tex <==
\begin{wraptable}{r}{8cm} 
\vspace{-1.0em}
  \centering
  \begin{tabular}{lccc}
    \toprule
    Platform & Train & Validation & Test \\
    \midrule
    Metaculus  & $1,576$ & $230$ & $275$ \\
    GJOpen  & $806$ & $161$ & $38$ \\
    INFER & $52$ & $50$ & $4$ \\
    Polymarket & $70$ & $229$ & $300$ \\
    Manifold   & $1,258$ & $170$ & $297$ \\
    \midrule
    \textbf{All Platforms} & $\mathbf{3,762}$ & $\mathbf{840}$ & $\mathbf{914}$ \\
    \bottomrule
  \end{tabular}
  \caption{\textbf{Distribution of our train, validation, and test sets across all 5 forecasting platforms.} Importantly, every question in the test set is from June 1, 2023 or later, after the training cut-off of our base LMs. Meanwhile, all questions in the train and validation sets were resolved before June 1, 2023, ensuring   no leakage from the tuning process.}
  \label{tab:curated-split}
  \vspace{-0.4em}
\end{wraptable}
% --

